Relaxing the Exclusion Restriction in Shift-Share Instrumental Variable Estimation

Many economic studies use shift-share instruments to estimate causal effects. Often, all shares need to fulfil an exclusion restriction, making the identifying assumption strict. This paper proposes to use methods that relax the exclusion restriction by selecting invalid shares. I apply the methods in two empirical examples: the effect of immigration on wages and of Chinese import exposure on employment. In the first application, the coefficient becomes lower and often changes sign, but this is reconcilable with arguments made in the literature. In the second application, the findings are mostly robust to the use of the new methods.

==> ADH-C.tex <==
\begin{tabular}{l*{7}{p{2cm} p{2cm} p{2cm} p{2cm} p{2cm} p{2cm} p{2cm} p{2cm}}}
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}\\
                    &\multicolumn{1}{c}{Original}&\multicolumn{1}{c}{ALasso}&\multicolumn{1}{c}{ALasso}&\multicolumn{1}{c}{CIM}&\multicolumn{1}{c}{CIM}&\multicolumn{1}{c}{AL AR}&\multicolumn{1}{c}{CIM AR}\\
\toprule
SSIV                &      -0.489&      -0.489&      -0.503&      -0.489&      -0.580&      -0.672&      -0.786\\
                    &    (0.0864)&    (0.0864)&    (0.0866)&    (0.0864)&     (0.112)&    (0.0769)&     (0.152)\\
F                   &       46.37&       46.37&       45.89&       46.37&       37.15&       80.77&       33.79\\
\midrule \# inv     &           0&           0&           1&           0&           8&          63&         128\\
Sign.               &           -&     0.01375&        0.05&     0.01375&        0.05&     0.01375&     0.01375\\
\bottomrule         \end{tabular}


==> wh_tsls_mult.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{\textwidth - 30\tabcolsep}{@{\hskip\tabcolsep\extracolsep\fill}l*{3}{C{2cm} C{2cm} C{2cm}}}
\midrule
\multicolumn{4}{c}{Wages (College or more)}\\ \midrule $\Delta m_{t}$&       0.877\sym{*}  &       1.249\sym{***}&      -0.494\sym{+}  \\
                    &     (0.343)         &     (0.367)         &     (0.297)         \\
\Delta m_{t-10}     &      -0.249         &      -0.709\sym{**} &       0.411\sym{+}  \\
                    &     (0.173)         &     (0.250)         &     (0.216)         \\
J                   &       38.47         &       41.72         &       30.55         \\
\midrule \# invalid &           0         &           2         &          11         \\
\end{tabular*}
}


==> wl_liml_mult.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{\textwidth}{@{\hskip\tabcolsep\extracolsep\fill}l*{3}{p{2cm} p{2cm} p{2cm} p{2cm}}}
\midrule
LIML                &       3.855         &       3.855         &      -1.240         \\
                    &     (10.04)         &     (10.04)         &     (0.807)         \\
L.LIML              &      -2.202         &      -2.202         &       0.964         \\
                    &     (5.946)         &     (5.946)         &     (0.596)         \\
F                   &      1453.3         &      1453.3         &       61.38         \\
\midrule \# inv     &           0         &           0         &           9         \\
Sign.               &           -         &           -         &     0.01302         \\
\bottomrule          \end{tabular*}


==> wl_shs_liml.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{\textwidth}{@{\hskip\tabcolsep\extracolsep\fill}l*{7}{p{2cm} p{2cm} p{2cm} p{2cm} p{2cm} p{2cm}}}
\midrule
LIML                &       0.306         &       0.306         &       0.717         &       0.306         &       0.717         &      -0.184         &      -0.405         \\
                    &     (0.370)         &     (0.370)         &     (0.400)         &     (0.370)         &     (0.400)         &     (0.499)         &     (0.349)         \\
F                   &       474.1         &       474.1         &       353.6         &       474.1         &       353.6         &       4.621         &       5.212         \\
\midrule \# inv     &           0         &           0         &           1         &           0         &           1         &           8         &           8         \\
Sign.               &           -         &        0.05         &        0.05         &         0.1         &         0.1         &     0.01302         &     0.01302         \\
\bottomrule          \end{tabular*}}


==> wl_shs_tsls.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{\textwidth}{@{\hskip\tabcolsep\extracolsep\fill}l*{7}{p{2cm} p{2cm} p{2cm} p{2cm} p{2cm} p{2cm}}}
\midrule \multicolumn{6}{c}{\textit{Panel C}: Change in avg. log weekly wages of low-skilled} \\ \midrule 2SLS&       0.252         &       0.252         &       0.575\sym{**} &       0.252         &       0.575\sym{**} &      -0.176         &      -0.403         \\
                    &     (0.153)         &     (0.153)         &     (0.204)         &     (0.153)         &     (0.204)         &     (0.488)         &     (0.348)         \\
F                   &       474.1         &       474.1         &       353.6         &       474.1         &       353.6         &       4.621         &       5.212         \\
\end{tabular*}
}


==> wl_ss_mult.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{\textwidth}{@{\hskip\tabcolsep\extracolsep\fill}l*{3}{p{2cm} p{2cm} p{2cm} p{2cm}}}
\midrule \multicolumn{6}{c}{\textit{Panel C}: Change in avg. log weekly wages of low-skilled} \\ \midrule SSIV&       0.411         &       0.411         &      -0.303         \\
                    &     (0.772)         &     (0.772)         &     (0.695)         \\
L.LIML              &      -0.366         &      -0.366         &     -0.0824         \\
                    &     (0.463)         &     (0.463)         &     (0.570)         \\
F                   &       0.282         &       0.282         &       0.714         \\
\end{tabular*}
}


==> wl_tsls_mult.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{\textwidth - 30\tabcolsep}{@{\hskip\tabcolsep\extracolsep\fill}l*{3}{C{2cm} C{2cm} C{2cm}}}
\midrule
\multicolumn{4}{c}{Wages (No Coll.)}\\ \midrule  $\Delta m_{t}$&       0.864\sym{**} &       0.864\sym{**} &      -0.278         \\
                    &     (0.273)         &     (0.273)         &     (0.183)         \\
\Delta m_{t-10}     &      -0.476\sym{***}&      -0.476\sym{***}&       0.222\sym{+}  \\
                    &     (0.124)         &     (0.124)         &     (0.126)         \\
J                   &       38.47         &       38.47         &       28.85         \\
\midrule \# invalid &           0         &           0         &           9         \\
Sign.               &           -         &     0.01302         &     0.01302         \\
\bottomrule          \end{tabular*} }

